Dynamics and Inference for Voter Model Processes

We consider a discrete-time voter model process on a set of nodes, each being in one of two states, either 0 or 1. In each time step, each node adopts the state of a randomly sampled neighbor according to sampling probabilities, referred to as node interaction parameters. We study the maximum likelihood estimation of the node interaction parameters from observed node states for a given number of realizations of the voter model process. In contrast to previous work on parameter estimation of network autoregressive processes, whose long-run behavior is according to a stationary stochastic process, the voter model is an absorbing stochastic process that eventually reaches a consensus state. This requires developing a framework for deriving parameter estimation error bounds from observations consisting of several realizations of a voter model process. We present parameter estimation error bounds by interpreting the observation data as being generated according to an extended voter process that consists of cycles, each corresponding to a realization of the voter model process until absorption to a consensus state. In order to obtain these results, consensus time of a voter model process plays an important role. We present new bounds for all moments and a bound that holds with any given probability for consensus time, which may be of independent interest. In contrast to most existing work, our results yield a consensus time bound that holds with high probability. We also present a sampling complexity lower bound for parameter estimation within a prescribed error tolerance for the class of locally stable estimators.

==> con-note.tex <==
\paragraph{*** These are some working notes}

Definition:
$$
\tilde{\Psi}_A = \min_{x\in \{0,1\}^n\setminus C}\frac{\E\left[\left|\sum_{u=1}^n\pi_u \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\right|\right]}{\min\{\pi^\top x, 1-\pi^\top x\}}.
$$

Related work:
\begin{itemize}
    \item \cite{HP02} 
    $$
    \EP[\tau] = O(M(G) \log(n))
    $$
    where $M(G)$ is the worst-case expected meeting time of two random walks on graph $G$.
    \item \cite{kanade}
    $$
    M = O\left(n d_{\max}\frac{1}{\Phi(G)}\log(d_{\max})\right).
    $$
    Combined with \cite{HP02},
    $$
    \EP[\tau] = \tilde{O}\left(n d_{\max}\frac{1}{\Phi(G)}\right).
    $$
    \item \cite{petra}
    $$
    \EP[\tau]=O\left(\frac{d(V)}{d_{\min}}\frac{1}{\Phi(G)}\right).
    $$
   
    \item \cite{CR16} 
    $$
    \EP[\tau] = O\left(\frac{1}{\Psi_A}\right)
    $$
    where $1/\Psi_A = (1/\pi^*)(1/\tilde{\Psi}_A)$.
    \item Our bound:
    $$
    \EP[\tau]\leq \frac{1}{\Phi_A}\log(1/(2\pi^*)).
    $$
    \item Other references: \cite{cox}, \cite{roberto}, \cite{fernley}
    \item \cite{roberto} gives a bound on the probability that a lazy random walk does not hit a moving target for a given number of steps in terms of maximum expected hitting time on $G$ (Theorem 1.3). Does this imply a bound on the probability tail distribution of consensus time by duality? Are there some known results on the probability tail bound of consensus time in literature (or other properties other than expected value)?
\end{itemize}


\noindent {\bf Claim:}
\begin{equation}
\frac{1}{\tilde{\Psi}_A} \leq \frac{2}{\Phi_A}.
\label{equ:psiphi}
\end{equation}

Proof:

\begin{eqnarray*}
&& \E\left[\left|\sum_{u=1}^n\pi_u \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\right|\right]\\
&\geq & \E\left[\left(\sum_{u=1}^n\pi_u \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\right)^2\right]\\
&=& \E\left[\sum_{u=1}^n\sum_{u'=1}^n \pi_u \pi_{u'} \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\left(x_u -\sum_{v'=1}^n Z_{u',v}x_{v'}\right)\right]\\
&=& \sum_{u=1}^n \pi_u^2 \E\left[\left(x_u-\sum_{v=1}^n Z_{u,v}x_v\right)^2\right] + \sum_{u=1}^n \sum_{u'\neq u} \pi_u \pi_{u'}\E\left[\left(x_u - \sum_{v=1}^n Z_{u,v}x_v\right)\right]\E\left[\left(x_{u'}-\sum_{v'=1}^n Z_{u',v'}x_{v'}\right)\right]\\
&=& \sum_{u=1}^n \pi_u^2 (x_u (1-a_u^\top x)+(1-x_u)a_u^\top x) + \sum_{u=1}^n \pi_u \pi_{u'}\sum_{u'\neq u} (x_u-a_u^\top x)(x_{u'}-a_{u'}^\top x)\\
&=& \sum_{u=1}^n \pi_u^2 (x_u (1-a_u^\top x)+(1-x_u)a_u^\top x) + \left(\sum_{u=1}^n \pi_u (x_u - a_u^\top x)\right)^2 - \sum_{u=1}^n 
\pi_u^2 (x_u -a_u^\top x)^2\\
&=& \sum_{u=1}^n \pi_u^2 (x_u (1-a_u^\top x)+(1-x_u)a_u^\top x) - \sum_{u=1}^n 
\pi_u^2 (x_u -a_u^\top x)^2\\
&=& \sum_{u=1}^n \pi_u^2 a_u^\top x(1-a_u^\top x).
\end{eqnarray*}

\begin{eqnarray*}
\frac{\E\left[\left|\sum_{u=1}^n\pi_u \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\right|\right]}{\min\{\pi^\top x, 1-\pi^\top x\}} & \geq & \frac{1}{2} \frac{\E\left[\left|\sum_{u=1}^n\pi_u \left(x_u -\sum_{v=1}^n Z_{u,v}x_v\right)\right|\right]}{\pi^\top x(1-\pi^\top x)}\\
&\geq & \frac{1}{2}\frac{\sum_{u=1}^n \pi_u^2 a_u^\top x(1-a_u^\top x)}{\pi^\top x (1-\pi^\top x)}.
\end{eqnarray*}

From this it follows $\tilde{\Psi}_A \geq \Phi_A/2$.


\noindent {\bf Claim}:

$$
\frac{1}{\tilde{\Psi}_A}\geq \frac{1}{2}\frac{1}{\Phi(G)}.
$$

\begin{eqnarray*} 
\E[|\pi^\top (I-Z)x|] &\leq &\sum_{u=1}^n \pi_u\E\left[\left|x_u -\sum_{v=1}^n Z_{u,v}x_v\right|\right]\\
&=& \sum_{u=1}^n \pi_u [x_u(1-a_u^\top x) + (1-x_u)(a_u^\top x)]\\
&=& \sum_{u=1}^n \sum_{v=1}^n (\pi_u a_{u,v} + \pi_v a_{v,u})x_u(1-x_v)
\end{eqnarray*}
where the inequality is by Jensen's inequality. 

$$
\sum_{u=1}^n \sum_{v=1}^n (\pi_u a_{u,v}+\pi_v a_{v,u}) x_u(1-x_v) = \frac{2}{d(V)}|E(S,S^c)|
$$
and 
$$
\min\{\pi^\top x, 1-\pi^\top x\} = \frac{1}{d(V)} \min\{d(S),d(S^c)\}.
$$
 
\noindent {\bf Claim:}

$$
\frac{1}{\Phi_A} \geq \frac{1}{4}\frac{1}{\Phi(G)}.
$$

This claim follows immediately from the previous two claims. 

\noindent {\bf Question:} $(1/\Phi_A)/(1/\Phi(G))\leq ?$. Does it hold $1/\Phi_A = O((d(V)/d_{\min})(1/\Phi(G)))$?

\begin{eqnarray*}
\frac{2}{d(V)}|E(S,S^c)| &=& \sum_{u=1}^n \sum_{v=1}^n (\pi_u a_{u,v}+\pi_v a_{v,u}) x_u (1-x_v)\\
&=& \sum_{u=1}^n \pi_u (x_u(1-a_u^\top x) + (1-x_u)(a_u^\top x))\\
&=& \sum_{u=1}^n \pi_u (a_u^\top (1-a_u^\top) + x_u = 2x_u a_u^\top x + (a_u^\top x)^2)\\
&=& \sum_{u=1}^n \pi_u a_u^\top x(1-a_u^\top x) + \sum_{u=1}^n\pi_u (x_u - a_u^\top x)^2.
\end{eqnarray*}

It follows
\begin{eqnarray*}
\frac{2}{d(V)}|E(S,S^c)| & \leq & c_A \frac{1}{\pi^*}\sum_{u=1}^n \pi_u^2 a_u^\top x (1-a_u^\top x)\\
&=& c_A \frac{1}{\pi^*} \frac{1}{d(V)^2}|E_2(S,S^c)|
\end{eqnarray*}
where
$$
c_A = 1 + \max_{x\in \{0,1\}^n\setminus C}\frac{\sum_{u=1}^n \pi_u (x_u-a_u^\top x)^2}{\sum_{u=1}^n \pi_u a_u^\top x(1-a_u^\top x)}.
$$

Hence, 
\begin{eqnarray*}
2 \frac{|E(S,S^c|}{\min\{d(S),d(S^c)\}} & \leq & c_A \frac{1}{d_{\min}}\frac{|E_2(S,S^c)|}{\min\{d(S),d(S^c)\}}\\
&\leq & c_A \frac{d(V)}{d_{\min}}\frac{|E_2(S,S^c)|}{d(S)d(S^c)}.
\end{eqnarray*}
Thus, we have
$$
2 \Phi(G) \leq c_A \frac{d(V)}{d_{\min}}\Phi_A,
$$
or, equivalently,
$$
\frac{1}{\Phi_A}\leq \frac{c_A}{2}\frac{d(V)}{d_{\min}}\frac{1}{\Phi(G)}.
$$

Q: $c_A \leq ?$. In the definition of $c_A$ we may relax the problem to optimization over $x\in [0,1]^n$ such that $\pi^\top x (1-\pi^\top x)\geq \pi^*/2$. 

Consider the case when $x = e_i$ where $e_i$ is the $i$-th basis vector. Then,
\begin{eqnarray*}
\sum_{u=1}^n \pi_u (x_u-a_u^\top x)^2 &=& \pi_i + \sum_{u=1}^n \pi_u a_{u,i}^2\\
&=& \frac{d_i}{d(V)} + \sum_{u=1}^n \frac{d_u}{d(V)}\frac{1}{d_u^2}\ind_{\{(u,v)\in E\}}\\
&=& \frac{1}{d(V)}\left(d_i + \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}}\right)
\end{eqnarray*}
and
\begin{eqnarray*}
\sum_{u=1}^n \pi_u a_u^\top x (1-a_u^\top x) &=& \sum_{u=1}^n \pi_u a_{u,i}(1-a_{u,i})\\
& = & \frac{1}{d(V)}\sum_{u=1}^n \left(1-\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}\\
& = & \frac{1}{d(V)}\left(d_i - \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}}\right).
\end{eqnarray*}

Thus, we have
$$
\frac{\sum_{u=1}^n \pi_u (x_u-a_u^\top x)^2 }{\sum_{u=1}^n \pi_u a_u^\top x (1-a_u^\top x)} = \frac{d_i + \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}}}{d_i - \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}}}.
$$

Note that 
$$
d_i - \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}} > 0
$$
as otherwise the graph has a bipartite component (a star subgraph) -- did we assume this? Hence, $d_u \geq 2$ for at least one neighbor of vertex $i$. It follows that 
$$
d_i - \sum_{u=1}^n \frac{1}{d_u}\ind_{\{(u,i)\in E\}} \geq \frac{1}{2}.
$$

We conclude
$$
\frac{\sum_{u=1}^n \pi_u (x_u-a_u^\top x)^2 }{\sum_{u=1}^n \pi_u a_u^\top x (1-a_u^\top x)} \leq 4 d_i \leq 4 d_{\max}.
$$

This does not look promising as we would like to have $c_A = O(1)$.

Here is another approach. 
\begin{eqnarray*}
|E(S,S^c)| & \leq & \frac{d(V)}{2} \left(\sum_{u=1}^n \pi_u a_u^\top x(1-a_u^\top x) + \sum_{u=1}^n\pi_u (x_u - a_u^\top x)^2\right)\\
& \leq & \tilde{c}_A \frac{|E_2(S,S^c)|}{2d(V)}  
\end{eqnarray*}
where 
$$
\tilde{c}_A = \min_{x\in \{0,1\}^n\setminus C} \left(\frac{\sum_{u=1}^n \pi_u a_u^\top x(1-a_u^\top x) + \sum_{u=1}^n\pi_u (x_u - a_u^\top x)^2}{\sum_{u=1}^n \pi_u^2 a_u^\top x(1-a_u^\top x)}\right). 
$$
It follows
$$
\frac{|E(S,S^c)|}{\min\{d(S),d(S^c)\}} \leq \frac{\tilde{c}_A}{2} \frac{|E_2(S,S^c))|}{d(S)d(S^c)}.
$$
Hence,
$$
\frac{1}{\Phi_A}\leq \frac{\tilde{c}_A}{2}\frac{1}{\Phi(G)}.
$$

Consider again $x=e_i$.
\begin{eqnarray*}
\frac{\sum_{u=1}^n \pi_u a_u^\top x(1-a_u^\top x)}{\sum_{u=1}^n \pi_u^2 a_u^\top x(1-a_u^\top x)} &=& d(V)\frac{\sum_{u=1}^n \left(1-\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}}{\sum_{u=1}^n \left(d_u-1\right)\ind_{\{(u,i)\in E\}}}\\
&\leq & d(V)\max_{u: (u,i)\in E} \frac{1-1/d_u}{d_u - 1}\\
&\leq & \frac{d(V)}{d_{\min}}.
\end{eqnarray*}

\begin{eqnarray*}
\frac{\sum_{u=1}^n \pi_u (x_u-a_u^\top x)^2 }{\sum_{u=1}^n \pi_u^2 a_u^\top x (1-a_u^\top x)} &=& d(V)\frac{\sum_{u=1}^n \left(1+\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}}{\sum_{u=1}^n (d_u - 1)\ind_{\{(u,i)\in E\}}}
\end{eqnarray*}

If all but one neighbour of $i$ have degree equal to $1$ (each such neighbor is connected only to $i$) and this one neighbour has degree $a > 1$, then,
$$
d(V)\frac{\sum_{u=1}^n \left(1+\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}}{\sum_{u=1}^n (d_u - 1)\ind_{\{(u,i)\in E\}}} = d(V) \frac{2(d_i-1)+1+1/a}{a-1}.
$$

This does not look good. 

For graphs such that $d_{\min}\geq 2$, we have
$$
d(V)\frac{\sum_{u=1}^n \left(1+\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}}{\sum_{u=1}^n (d_u - 1)\ind_{\{(u,i)\in E\}}} \leq 2\frac{ d(V)}{d_{\min}-1}\leq 4\frac{d(V)}{d_{\min}}
$$
which is good. The condition $d_{\max}\geq 2$ holds for graphs such as complete graph with $n\geq 3$ and cycle with $n\geq 3$.

For all graphs except for a star, we have
$$
d(V)\frac{\sum_{u=1}^n \left(1+\frac{1}{d_u}\right)\ind_{\{(u,i)\in E\}}}{\sum_{u=1}^n (d_u - 1)\ind_{\{(u,i)\in E\}}} \leq 2d(V)d_{\max} 
$$
which is $O(d(V))$ for constant-degree graphs. For example, this applies to a path with $n\geq 4$ vertices. 

The above considerations are only for $x$ being a basis vector, i.e. $x$ is such that exactly one node is in state $1$ and other nodes are in state $0$. They indicate cases when we cannot have $\tilde{c}_A = O(d(V)/d_{\max})$ or $\tilde{c}_A = O(d(V))$. Indeed, for bounding $\tilde{c}_A$ one would need to consider all $x\in \{0,1\}^n \setminus C$.


Consider the case where $A$ has elements given by
$$
a_{u,v} = \frac{1}{2}\ind_{\{u=v\}} + \frac{1}{2}\frac{1}{d_u}\ind_{\{(u,v)\in E\}}.
$$
In this case, we have $\pi_u = d_u/d(V)$, for $u\in V$.

Furthermore, we have
\begin{eqnarray*}
\sum_{u\in V} \pi_u^2 a_u^\top x (1-a_u^\top x) &=& \frac{1}{4d(V)^2} \sum_{u\in V} (d_u \ind_{\{u\in S\}} + d_u(S))(d_u \ind_{\{u\in S^c\}}+d_u(S^c))\\
&\geq & \frac{d_{\min}}{4d(V)^2}\left(\sum_{u\in S} d_u(S^c) + \sum_{u\in S^c }d_u(S)\right)\\
&=& \frac{d_{\min}}{2 d(V)^2}|E(S,S^c)|.
\end{eqnarray*}
It follows
\begin{eqnarray*}
\frac{\sum_{u\in V}\pi_u^2 a_u^\top x(1-a_u^\top x)}{\pi^\top x(1-\pi^\top x)} & \geq & \frac{d_{\min}}{2}\frac{|E(S,S^c)|}{d(S)d(S^c)}\\
&\geq & \frac{d_{\min}}{2d(V)} \frac{|E(S,S^c)|}{\min\{d(S),d(S^c)\}}.
\end{eqnarray*}

Hence, we have
$$
\frac{1}{\Phi_A}\leq 2\frac{d(V)}{d_{\min}}\frac{1}{\Phi(G)}.
$$

\paragraph{*** end of working notes}

==> conc.tex <==
tbd

==> numerical.tex <==
tbd

==> related.tex <==
There is a large body of research on representing, measuring and learning from social and economic networks, e.g. see \cite{Jackson2008} for a book exposition. Several models have been used to study opinion formation and consensus in networks. One of the most influential models is by \cite{D74} introduced to study how consensus is reached by individuals in a network, when individual opinions are updated according to their neighbours' average opinions. In this model, each individual has possibly different weights associated with links to its neighbors and the opinions are represented by real-valued variables. For the voter model we study, it has a different updating rule of the individual opinions, where each individual randomly selects one of its neighbours and adopts the observed opinion, which is measured by discrete binary variables. 

Threshold models of collective behavior was proposed by \cite{G78} to study the formation of binary opinions in a group. It assumes that each individual updates its state according to a threshold update rule, adopting a new state if the number of neighbors in this state exceeds the threshold. 

\cite{KY14} studied the factors that affect the speed of the innovation in a network and the time to reach a majority opinion under a local interaction model.

\cite{BHW92} provides conditions that will make a cascade almost sure start, but also showed the information cascades can be used to explain the conformity and the spread of the behaviours. It claims that most of individuals will automatically ignore its own belief according the history of information available. Therefore, small amount of modification on the information will affect the spread of cascade largely due to the fragile behaviors of the conformists.

\cite{HP02} studied a voter model whose definition correspond to the model studied in our paper. They established a precise characterization of the hitting probabilities of a consensus state, in which either all nodes are in state $0$ or all nodes are in state $1$. Our work extends this line of work by providing results on the consensus time, specifically, providing a bound on the expected consensus time and a concentration bound for a sum of consensus times of independent voter model processes. 

\cite{CR16} studied a class of linear voter models which subsumes the voter model studied in our work as a special case. They established closed-form expressions for the hitting probabilities of the the consensus states, and an upper bound on the expected consensus time. Our work extends this line of work by providing a new upper bound on the expected consensus time, which we have shown to be tighter, and providing also probability tail bounds. 

\cite{CDFR18}

If the states of vertices are initially distinct, the voter process takes $\Theta(n)$ expected steps to reach consensus on many classes of expander graphs on $n$ vertices. 

\cite{CEOR13} established bounds on the expected consensus time for the voter process on general connected graphs based on the eigenvalue gap and variance of the degree sequence. Specifically, for a graph $G$ with $n$ vertices, they found a bound on the expected consensus time $O(n / (\mu (1-\lambda))$ where $\lambda$ is the second largest eigenvalue in absolute value of the transition matrix of a simple random walk on $G$, and $\mu = (1/n)\sum_{v\in V} d(v)^2 / ((1/n)\sum_{v\in V}d(v))^2$.

\cite{BGKM16} 

Similar problem was studied in \cite{PH15} for a general model of cascades with observations consisting of node states up to a given time. \cite{HC19} also considered estimation of node interaction rates from observations consisting of either infection times or infection state of nodes. This work assumed that the properties of the infection spread is not perfectly known, unlike to \cite{NS12} and \cite{PH15}. 

\cite{MB16} studied a structured vector auto-regression estimation problem, obtaining sample complexity and non-asymptotic estimation error bounds and showing that the estimation error is of the same order as the one for a Lasso-type regression estimator under independent samples.

\cite{HRW19}

\cite{basu2015}

\cite{CS77}

\cite{LWZ18} also \cite{ZLWZ19}

\cite{HRW16} studied the inference of network parameters for a vector autoregressive model according to a generalized linear model. Specifically, they considered maximum likelihood estimation under a sparsity constraint, and derived an upper bound for the Frobenius-norm estimation error. This model accommodates a Bernoulli autoregressive process, which bears a similarity with the noisy voter model. More recently, \cite{SparseBer2019} studied the parameter estimation for Bernoulli autoregressive processes with lag parameter $p\geq 1$ in a high dimensional setting. The framework used by \cite{HRW16} and \cite{SparseBer2019} can not be directly applied to study the parameter estimation problem for the voter model because it is developed for ergodic stochastic processes. 

\cite{NVR17} studied a network vector autoregressive model of opinion formation in a social network, which assumes a random intercept term and symmetric regression coefficients. \cite{ZP18} relaxed these symmetry assumptions by studying a grouped network vector autoregression model. Both these papers studied an ordinary least-squares type estimator and derived its asymptotic properties. More general models were studied by \cite{SMTJR18} and \cite{JP19}. %In our model, we assume that each node will react differently to each of its neighbour and non-iid noise process is used.

\cite{SMTJR18} studied a discrete-time linear system identification problem with additive Gaussian noise, and established lower and upper bounds of the operator-norm estimation error of the ordinary least-squares estimator. \cite{JP19} established sampling complexity lower and upper bounds. We adapted their framework for deriving a lower bound for problem, which amounts to studying random linear systems with i.i.d. matrices of random linear transformations. 

\cite{MRW19} used the Poisson process to count the number of events at a node during a certain period of time using the history events of all it neighbours. Parameter estimation of interaction matrix $A$ is also studied here together with the upper bound of the estimation error in the Frobenius norm. In our model, we consider the similar inference problem but model each of the individuals' decision on a certain event via the Bernoulli process.

\cite{MRW19b} studied parameter estimation problem for the multivariate Bernoulli autoregressive (BAR) when the data can be only partially observed. They proposed a novel method to estimate the parameters using an unbiased estimator from the log-likelihood function with complete data and both the statistical error and the optimisation error are characterised.

\cite{Trace13} studied the network inference problem on reconstructing the edge set of a network from the given chronology of the infection times (traces). A sample complexity lower bound on the number of traces needed is derived using First-Edge Algorithm. The cascade model studied in \cite{Trace13} is different from the one we studied, the cascade model they studied is with continuous time and it does not constrain the length of time that a node can remain infected. They assume that each node will pick and infect each of its neighbours with a probability constant $p$, the infected neighbour will remain active after a countdown, the length of the countdown is according the Exp($\lambda$) distribution with $\lambda$ is known. Whereas, in our model, we assume each node will have different probability weights to interact with its neighbours and pass the infection. Both \cite{Trace13} and our work consider the Maximum likelihood estimation (MLE).

\cite{Diff16} studied the network structure recovery problem of the continuous-time diffusion model. A $\ell_1$- regulator is used together with maximum likelihood estimation (MLE) using the infection time of each nodes in the network. The corresponding sample complexity is derived. (Maybe I need to add the actual number of the sample complexity here, and compare it with \cite{Trace13},\cite{NS12} and our result.)
